A Triple Rollover: A third multiply-imaged source at z~6 behind the Jackpot gravitational lens

UUsing a five-hour adaptive-optics-assisted observation with MUSE, we have identified a doubly-imaged Ly alpha source at redshift 5.975 behind the z=0.222 lens galaxy J0946+1006 ('the Jackpot'). The source separation implies an Einstein radius of ~2.5 arcsec. Combined with the two previously-known Einstein rings in this lens (radii 1.4 arcsec at z = 0.609 and 2.1 arcsec at z ~ 2.4), this system is now a unique galaxy-scale triple-source-plane lens. We show that existing lensing models for J0946+1006 successfully map the two new observed images to a common point on the z=5.975 source plane. The new source will provide further constraints on the mass distribution in the lens and in the two previously known sources. The third source also probes two new distance scaling factors which are sensitive to the cosmological parameters of the Universe. We show that detection of a new multiply imaged emission-line source is not unexpected in observations of this depth; similar data for other known lenses should reveal a larger sample of multiple-image-plane systems for cosmography and other applications.

==> oldstufflongsincecut.tex <==

As reviewed in the introduction, lenses with multiple source planes can find application in geometric tests of cosmological parameters, and in providing multiple tracers for the mass distribution in galaxies. 

In the case of \jj, the configuration of the two Einstein rings 
was already fairly favourable, and so it possible that adding the $z$\,=\,5.975 lens plane in \jj\ brings little marginal gain to such analyses. (Certainly the $w$ effect pretty much saturates by z=3.)  The new source however has the advantage of a secure spectroscopic redshift, so that a two-plane analysis of the $z$\,=\,0.609 and $z$\,=\,5.975 can bypass the uncertain redshift of the intermediate plane. On the other hand, the contribution of the redshift uncertainty to the cosmological inference is ??? (not huge?). Moreover it is still necessary to include the deflections induced by the second source, which also depend on its uncertain redshift. 

{\it NB: I have looked at MUSE spectra combined over pixels which should correspond to the second source, but cannot find any features that might secure a redshift. IR data from ERIS would be really useful here.}


\section{Projected Mass Profile}

{\it Might be nice to provide a ``dumb-but-easily-visualised'' lensing-mass profile.  Can start with the most naive projected mass estimates, then include reasonable estimates for compound lensing etc, informed by more sophisticated modelling.}

For a standard single source-plane system, lensing provides a robust estimate of the mass projected within the critical curve.  Under circular symmetry, this is simply the mass within the Einstein radius.   Where sufficient constraints are present, e.g. for quadruply-imaged sources, corrections for ellipticity and external shear can be determined.

In principle, each source plane in the Jackpot lens should yield its own Einstein mass at a given radius, allowing us to construct the projected mass profile over radii 1.4--2.5\,arcsec, corresponding to 5--9\,kpc at $z$\,=\,0.222. This scale is expected to be close to the transition from the stellar dominated regime in the inner regions to the zone where dark-matter dominated the projected mass.

In practice, the effects of compound lensing need to be taken into account to derive the projected mass from S2 and S3. Also S3 seems to be approximately along the expansive axis of the shear, so this needs to be corrected for as well. ({\it Though presumably we can't strictly assume the shear for S3 is the same as that derived in the fitting of S1/S2.})




\section{Cosmology solved}\label{sec:cosmo}

Fitting lensing models to all three three source planes; we find ... ({\it Tom to fill in a few details}) ... and hence all relevant cosmological parameters are determined at the $<$0.1 per cent level, and cosmology is solved.






\section{Summary and outlook}\label{sec:outlook}

{\it Preview a few science applications for this lens but beyond scope of current report, e.g.:

\begin{itemize}

\item
Cosmology constraints from more sophisticated modelling?

\item
Mass profile from multiple source planes (ref to Sonnenfeld, etc). IMF and DM halo. (If we infer a naive projected mass within 2.5\,arcsec from the new source, that mass looks quite quite compared to the other two constraints? Yields too abrupt a change to be reproduced from mass-follows-light plus NFW halo. Of course this ignores compound lensing effects but might expect to be small -- see below). 

\item
Multi-plane lensing constraints on the intermediate-redshift sources?  (But given the z=6 source must be quite off-axis, and the ring sources on-axis, perhaps the compound lensing effects can be expected to be small?)


\end{itemize}



\begin{figure}
\vskip 0mm
\includegraphics[width=85mm]{projprof.pdf} 
\vskip 1mm
\caption{Projected mass profile, from the three sources. Einstein radii are taken from the fit of \ca\ for S1, ?? for S2. 
For S2 and S3, we apply a correction of 0.16\,arcsec deflection from the S1 plane ({\it but is this at all correct?}). For S3 we also take into account the shear estimated by \ca. The solid lines show a stars+DM model in which the halo is of the NFW form and the stars follow the luminosity profile from S+12. The dashed lines assume a radial gradient in mass-to-light ratio, with a slope of --0.25 as in S+18.}\label{fig:projprof}
\end{figure}

}


Looking beyond applications of \jj\  
specifically, our discovery suggests that a programme of deep IFU observations for known lenses could reveal additional faint lensed sources in other systems, and hence establish a meaningful {\it sample} of double source-plane lenses for cosmology and other applications.
\ca\ estimated that a competitive determination of $w$ could be obtained from a sample of just six suitably-configured DSPLs. 

For galaxies that are not known to be lenses at all, our result supports the closing remarks of \citet{2015MNRAS.449.3441S},
that `strongly lensed background line emitters could be detected for any chosen massive elliptical' given IFU observations of sufficient depth. In this context, we note that the sensitivity of our current MUSE data should be reached in less than 15\,minutes integration with the 39m E-ELT. 





\begin{figure}
\vskip 0mm
\includegraphics[width=85mm]{emisscounts.pdf} 
\vskip 1mm
\caption{Empirical source counts from the MUSE Hubble Ultra Deep Field observations, converted to average number of multiply-images sources 
behind \jj\ as a function of emission-line flux. The counts assume a constant Einstein radius and hence a constant cross-section for multiple imaging. Fluxes have been boosted by a factor of three (the average lensing amplification for the brighter image for a SIS lens; Tom to check).
No correction has been made for increased noise due to the foreground continuum from the lens. 
{\bf Obsolete: retained for now, for comparison to following figure.}
}\label{fig:emisscounts}
\end{figure}


% Some stuff cut from the inteo

For both cosmological and galaxy structure  applications, the optimal DSPL configuration is that in which the first source is close behind the primary lens, while the second is much more distant. 
By happy (partial) coincidence the first 
DSPL system to be discovered, fulfils these criteria. 
The `Jackpot' lens \jj\ was discovered as part of the SLACS (Sloan Lens ACS) survey ({\it go back and check refs and timeline.}) The primary lens is at $z_{\rm l}$\,=\,0.222 while the bright source detected in the SDSS spectrum is at $z_{\rm s,1}$\,=\,0.609 and forms arcs with an Einstein radius $\theta_{Ein,1}$\,$\approx$\,?.?\,arcsec. HST observations
revealed a second system of arcs at $\theta_{Ein,2}$\,$\approx$\,?.?\,arcsec. 
The larger Einstein radius implies a more distant source, but only a photometric redshift estimate has yet been obtained $z_{\rm s,2}$\,=\,2.4$^{+??}_{-??}$ \citep{2012ApJ...752..163S}.
From the DSPL analysis combined with a CMB prior, \ca\ derived $w$\,=\,--1.17$\pm$0.20 from this system alone. ({\it Need more detailed summary of the analysis.})


% old version of source table
\begin{table}
\caption{MUSE detected emission-line sources within 8\,arcsec from \jj. The positions of the doubly-imaged source are given first, followed by six singly-imaged sources U1--U6. Only the first two of these
have secure redshifts. The remainder have only a single line detection, and we tabulate the corresponding redshift for Ly\,$\alpha$. However unlike in the images of S3, the line cannot be confidently identified from its profile in these faint sources. {\it Coords for the extra sources ought to be refined on narrow-band centroids, for what it's worth. And would be good to quote brightest line flux. And verify pipeline flux calibration. Include S3A, S3B, but not S1 since the position is ill-defined}}\label{tab:othersources}
    \centering
    \begin{tabular}{lccccl}
    \hline
    ID & $\Delta$RA & $\Delta$Dec & sep & $z$ &  notes \\ß
        \hline
        S3A & & & & 5.975 & Ly\,$\alpha$ \\
        S3B & & & & 5.975 & Ly\,$\alpha$ \\
        \hline
        U1 & --4.0 & --0.2 & 4.0 & 0.395 & [O\,{\sc ii}], [O\,{\sc iii}], H$\alpha$ \\ % & OIII/Halpha k=1829/3565 $z$\,=\,0.395 4.0         \,arcsec; HST detectn?\\
        U2 & +6.0 & --1.6 & 6.2 & 1.346 & [O\,{\sc ii}] \\ %& k=3234 OII at $z$\,=\,1.346, 6.2\,arcsec\\
        U3 & +4.0 & +2.6 & 4.8 & (3.51?) & single line \\ %&  single line k=623 (Ly\,$\alpha$ at $z$\,=\,3.508?) $\sim$4.8\,arcsec \\
        U4 & --2.2 & +4.0 & 4.5 & (4.77?) & single line \\ %& single line k=1847 (Ly\,$\alpha$ at U4 & $z$\,=\,4.767?) 4.5\,arcsec \\
        U5 & +3.4 & +5.8 & 6.7 & (5.05?) & single line \\% k=2118 single line (Ly$\alpha$	at $z$\,=\,5.046?) 6.7\,arcsec\\
        U6 & +2.8 & --5.2 & 5.9 & (5.72?) & single line \\% k=2776 single line (Ly$\alpha$	at $z$\,=\,5.723?) 5.9 arcsec\\
    % further out:
        % 78& 64 & k=2116 OII at $z$\,=\,0.972,  8.7\,arcsec\\
        % 16 & 4 & multiple lines at $z$\,=\,0.395 8.9\,arcsec; HST detn  \\
    \hline
    \end{tabular}
\end{table}

% table from before Mar 31



\begin{table}
\caption{MUSE-detected emission-line sources within 8\,arcsec from \jj. The positions of the doubly-imaged source are given first, followed by six singly-imaged sources U1--U6. Only the first two of these have secure redshifts. Sources U3--U6 have only a single line detection, and we tabulate the corresponding redshift for Ly\,$\alpha$. However unlike in the images of S3, the line cannot be confidently identified from its profile in these faint sources.}\label{tab:othersources}
    \centering
    \begin{tabular}{lcccccc}
    \hline
    ID & $\Delta$RA & $\Delta$Dec & sep & flux & line & $z$ \\
    %& arcsec & arcsec & arcsec & \cgsflux & \\
    \hline
%+3.04 -1.91 +3.59 7.60+/-0.58 8475 3021 5.976 5.976
%-1.00 +0.87 +1.32 5.32+/-0.42 8476 3022 5.976 5.976
S3A & +3.04 & --1.91 & 3.59 & \z7.60$\pm$0.58 & Ly\,$\alpha$ & 5.975 \\
S3B & --1.00 & +0.87 & 1.32 & \z5.32$\pm$0.42 & Ly\,$\alpha$ & 5.975 \\
\hline
U1 & --4.02 & +0.09 & 4.03 & \z1.33$\pm$0.22 & [O\,{\sc iii}] & 0.395 \\
U2 & +5.71 & --1.25 & 5.85 & 13.69$\pm$0.67 & [O\,{\sc ii}] & 1.347 \\
U3 & +4.06 & +2.71 & 4.89 & \z2.16$\pm$0.41 & Ly\,$\alpha$? & 3.51? \\
U4 & --2.13 & +3.94 & 4.48 & \z4.97$\pm$0.20 & Ly\,$\alpha$? & 4.77? \\
U5 & +3.54 & +5.89 & 6.87 & \z2.66$\pm$0.39 &  Ly\,$\alpha$? & 5.05? \\
U6 & +3.17 & --5.19 & 6.08 & \z2.34$\pm$0.19 &  Ly\,$\alpha$? & 5.72? \\
    \hline
%-4.02 +0.09 +4.03 1.33+/-0.22 6985 1829 0.395 0.395
%-2.15 +3.94 +4.49 5.39+/-0.14 7008 1848 4.768 4.768
%+3.04 -1.91 +3.59 7.60+/-0.58 8475 3021 5.976 5.976
%-1.00 +0.87 +1.32 5.32+/-0.42 8476 3022 5.976 5.976
\end{tabular}
\end{table}

